Discrete Hashing with Deep Neural Network

This paper addresses the problem of learning binary hash codes for large scale image search by proposing a novel hashing method based on deep neural network. The advantage of our deep model over previous deep model used in hashing is that our model contains necessary criteria for producing good codes such as similarity preserving, balance and independence. Another advantage of our method is that instead of relaxing the binary constraint of codes during the learning process as most previous works, in this paper, by introducing the auxiliary variable, we reformulate the optimization into two sub-optimization steps allowing us to efficiently solve binary constraints without any relaxation. The proposed method is also extended to the supervised hashing by leveraging the label information such that the learned binary codes preserve the pairwise label of inputs. The experimental results on three benchmark datasets show the proposed methods outperform state-of-the-art hashing methods.

==> not_use/experiment.tex <==
\section{Evaluation of Unsupervised Discrete Hashing with Deep Neural Network}
This section presents results of UDH-DNN. We compare UDH-DNN with following state-of-the-art unsupervised hashing methods: Spectral Hashing (SH)~\cite{DBLP:conf/nips/WeissTF08},  
%Semantic Hashing (SeH)~\cite{DBLP:SeH}, AnchorGraph Hashing (AGH)~\cite{DBLP:conf/icml/LiuWKC11}, 
Iterative Quantization (ITQ)~\cite{DBLP:conf/cvpr/GongL11}, Binary Autoencoder (BA)~\cite{Carreira-Perpinan_2015_CVPR}, Spherical Hashing (SPH)~\cite{CVPR12:SphericalHashing}, K-means Hashing (KMH)~\cite{DBLP:conf/cvpr/HeWS13}.
\subsection{Dataset and evaluation protocol}
\paragraph{CIFAR-10}  CIFAR-10~\cite{Krizhevsky09} contains 60,000 color images in 10 classes. Each image has size of $32\times 32$. Training set contains 50,000 images and the testing set contains 10,000 images. In this experiment, we ignore the class labels. As standardly done in the literature~\cite{DBLP:conf/cvpr/GongL11,Carreira-Perpinan_2015_CVPR}, we extract $D = 320$ GIST features~\cite{gist} from each image.
%\paragraph{NUS-WIDE} NUS-WIDE~\cite{nus-wide-civr09} dataset contains 269,648 images collected from Flickr. The training set contains 161,789 images and the testing set contains 107,859 images. The provided 128-dimensional wavelet features features are used. 
\paragraph{MNIST} The MNIST~\cite{mnistlecun} dataset consists of 70,000 handwritten digit
images from 10 classes (labeled from 0 to 9). The training set contains 60,000 samples, and the test set contains 10,000 samples. The size of each image is $28\times28$. Each image was represented as a 784-D gray-scale feature vector by using its intensity. 
\paragraph{SIFT1M} SIFT1M~\cite{herve_pami2011} dataset contains 128-dimensional SIFT vectors. This is standard dataset used for evaluating large scale approximate nearest neighbor search.  There are 1M vectors for indexing; 100K vectors for training (separated from indexing set) and 10K vectors for testing. 
\paragraph{Evaluation metric} 
We follow standard setting widely used in unsupervised hashing~\cite{DBLP:conf/cvpr/GongL11,Carreira-Perpinan_2015_CVPR}, i.e., using Euclidean neighbors, to create ground truth for queries. Follow~\cite{Carreira-Perpinan_2015_CVPR}, for each query, we find $50$ its Euclidean nearest neighbors and use these nearest neighbors as ground truth. We used the following evaluation metrics~\cite{DBLP:conf/cvpr/GongL11,Carreira-Perpinan_2015_CVPR} to measure the performance of methods. 1) mean average precision (mAP) which not only considers precision but also considers rank of retrieval results; %2) precision when $K$ nearest neighbors are returned (precision$@K$); 3) precision of Hamming radius $r$ (precision$@r$) which measure precision on retrieved images having Hamming distance to query $\le r$ (if no images satisfy, we report zero precision). 
 2) precision of Hamming radius $r$ (precision$@r$) which measure precision on retrieved images having Hamming distance to query $\le r$ (if no images satisfy, we report zero precision).  
\paragraph{Implementation note}
In our deep model, we use $n=5$ layers (including input and output layer). The activation function for layers $2$ and $3$ are sigmoid function; for layers $4$ and $5$ are linear activation functions. The parameters $\lambda_1$, $\lambda_2$, $\lambda_3$ and $\lambda_4$ were empirically set as $10^{-5}$, $5\times 10^{-2}$, $10^{-2}$ and $10^{-6}$, respectively. For the CIFAR-10 and MNIST datasets, the number of units in hidden layers $2,3,4$ were empirically set as $[90 \to 20 \to 8]$, $[90 \to 30 \to 16]$, $[120 \to 50 \to 32]$  and $[160 \to 110 \to 64]$ for the 8, 16, 32 and 64 bits respectively.

For the SIFT1M dataset, the number of units in hidden layers $2,3,4$ were empirically set as 
$[90 \to 20 \to 8]$, $[90 \to 30 \to 16]$, $[100 \to 50 \to 32]$  and $[100 \to 80 \to 64]$ for the 8, 16, 32 and 64 bits respectively.

\subsection{Retrieval results}
%\subsection{Results on CIFAR-10}
\begin{figure*}[!t]
\centering
\subfigure[]{
       \includegraphics[scale=0.35]{cifar10_mapK.pdf}
       \label{fig:cifar_mAP}
}
%\subfigure[]{
%       \includegraphics[scale=0.35]{cifar10_pK.pdf}
%       \label{fig:cifar_pK}
%}
\subfigure[]{
       \includegraphics[scale=0.35]{cifar10_pr3.pdf} 
       \label{fig:cifar_pr3}
}
\subfigure[]{
       \includegraphics[scale=0.35]{cifar10_pr4.pdf} 
       \label{fig:cifar_pr4}
}
%\caption[]{Comparative evaluation on CIFAR-10 dataset. \ref{fig:cifar_pK} and ~\ref{fig:cifar_mAP}: Precision and mAP when considering top 50 returned nearest neighbors.~\ref{fig:cifar_pr}: Precision when considering images with in Hamming distance 2.}
\caption[]{Comparative evaluation on CIFAR-10 dataset.~\ref{fig:cifar_mAP}: mAP.   \ref{fig:cifar_pr3} and \ref{fig:cifar_pr4}: Precision when considering images with in Hamming distance 3 and 4, respectively.}
\label{fig:cifar10}
\end{figure*}

\paragraph{Results on CIFAR-10 dataset} Figure~\ref{fig:cifar10} shows retrieval results of different methods with different code lengths $L$ on CIFAR-10 dataset. 

In term of mAP, the proposed UDH-DNN achieves the best results for all code lengths. The improvement is more clear at high $L$. The mAP of UDH-DNN consistent outperforms binary autoencoder (BA)~\cite{Carreira-Perpinan_2015_CVPR} which is current state-of-the-art unsupervised hashing method. 

When precision of Hamming radius $r$ is used, the following observations are consistent for both $r=3$ and $r=4$. The UDH-DNN is comparable to other methods at low $L$ (i.e. $L = 8, 16$). At $L = 32$, UDH-DNN significant outperforms other methods. When $L = 64$, all methods decrease the precision. The reason is that many query images have no neighbors at a Hamming distance of $r$ or less and we report zero precision for those cases. The precision of UDH-DNN is lower than some compared methods at $L=64$. However, we note a larger variance: the highest precision is achieved by UDH-DNN at $L=32$ for both $r=3$ and $r=4$ cases.

\paragraph{Results on MNIST dataset} Figure~\ref{fig:mnist} shows retrieval results of different methods with different code lengths $L$ on MNIST dataset. 

The results are quite consistent with the results on the CIFAR-10 dataset. The proposed UDH-DNN achieves the best mAP for all code lengths. The mAP improvement is more clear at high $L$.

When precision of Hamming radius $r$ is used, all methods achieve similar precision at low $L$ ($L=8, 16$). At $L=32$, UDH-DNN outperforms other methods by a fair margin.
When $L$ is large, i.e. $L = 64$, except for ITQ which slightly increase precision at $r=4$, all methods decrease the precision. The precision of UDH-DNN is lower than some compared methods at $L=64$. However, it is worth noting that the highest precision is achieved by UDH-DNN at $L=32$ for both $r=3$ and $r=4$ cases.

\begin{figure*}[!t]
\centering
\subfigure[]{
       \includegraphics[scale=0.35]{mnist_mapK.pdf}
       \label{fig:mnist_mAP}
}
%\subfigure[]{
%       \includegraphics[scale=0.35]{mnist_pK.pdf}
%       \label{fig:mnist_pK}
%}
\subfigure[]{
       \includegraphics[scale=0.35]{mnist_pr3.pdf} 
       \label{fig:mnist_pr3}
}
\subfigure[]{
       \includegraphics[scale=0.35]{mnist_pr4.pdf} 
       \label{fig:mnist_pr4}
}
\caption[]{Comparative evaluation on MNIST dataset.~\ref{fig:cifar_mAP}: mAP.   \ref{fig:cifar_pr3} and \ref{fig:cifar_pr4}: Precision when considering images with in Hamming distance 3 and 4, respectively.}
\label{fig:mnist}
\end{figure*}


\begin{figure*}[!t]
\centering
\subfigure[]{
       \includegraphics[scale=0.35]{sift1m_mapK.pdf}
       \label{fig:sift1m_mAP}
}
\subfigure[]{
       \includegraphics[scale=0.35]{sift1m_pr3.pdf} 
       \label{fig:sift1m_pr3}
}
\subfigure[]{
       \includegraphics[scale=0.35]{sift1m_pr4.pdf} 
       \label{fig:sift1m_pr4}
}
\caption[]{Comparative evaluation on SIFT1M dataset.~\ref{fig:sift1m_mAP}: mAP.   \ref{fig:sift1m_pr3} and \ref{fig:sift1m_pr4}: Precision when considering images with in Hamming distance 3 and 4, respectively.}
\label{fig:sift1m}
\end{figure*}
\paragraph{Results on SIFT1M dataset} Figure~\ref{fig:sift1m} shows retrieval results of different methods with different code lengths $L$ on MNIST dataset. As computing mAP is slow on this large dataset, we consider top-$50,000$ returned neighbors when computing mAP. 

In term of mAP, the results is consistent as results on CIFAR-10 and MNIST dataset. We can see that the proposed UDH-DNN clearly outperforms the other compared methods at high $L$.   

\textcolor{red}{Rerun our UDH-DNN and ITQ for case L=64}

==> related_work.tex <==
\section{Related Work}

